What's Wrong? Refining Meeting Summaries with LLM Feedback

Meeting summarization has become a critical task since digital encounters have become a common practice. Large language models (LLMs) show great potential in summarization, offering enhanced coherence and context understanding compared to traditional methods. However, they still struggle to maintain relevance and avoid hallucination. We introduce a multi-LLM correction approach for meeting summarization using a two-phase process that mimics the human review process: mistake identification and summary refinement. We release QMSum Mistake, a dataset of 200 automatically generated meeting summaries annotated by humans on nine error types, including structural, omission, and irrelevance errors. Our experiments show that these errors can be identified with high accuracy by an LLM. We transform identified mistakes into actionable feedback to improve the quality of a given summary measured by relevance, informativeness, conciseness, and coherence. This post-hoc refinement effectively improves summary quality by leveraging multiple LLMs to validate output quality. Our multi-LLM approach for meeting summarization shows potential for similar complex text generation tasks requiring robustness, action planning, and discussion towards a goal.

==> figures/callables/RQ2_template_result.tex <==
\begin{figure}[t]
  \includegraphics[width=1\linewidth]{figures/_storage/image-20240404-071504.png}
  \caption {(EXAMPLE) A diagram showing how well mistake-finding with LLMs works. The dotted line shows the naïve approach of always labeling samples as incorrect, which gives an accuracy of X.}
   \label{fig:RQ1_sample_result}
\end{figure}


==> figures/callables/RQ4_sample_result.tex <==
\begin{figure}[t]
  \includegraphics[width=1\linewidth]{figures/_storage/image-20240404-074356.png}
  \caption {An example of how the result can be processed and visualized.}
   \label{fig:RQ4_sample_result}
\end{figure}


==> figures/callables/refinement_illustration_intro.tex <==
\begin{figure}[h!]
  \includegraphics[width=0.99\linewidth]{figures/_storage/Overview.png}
  \caption {(PLACEHOLDER) Illustration of improving summarization utilizing both positive and negative feedback. The summarization agent refines its output by correcting the pointed-out mistakes.}
   \label{fig:RQ1_sample_result}
\end{figure}


==> text/archive/04_methodology.tex <==
\subsection{Error identification approach}
% We use as main model GPT-4 Turbo version XXXXXXX.
The feedback models are tasked to identify the derived error types.
The feedback models are prompted with the same prompt structure:

Since the evaluator is not fine-tuned with supervised data or trained reinforcement learning rewards, we follow recent studies to guide the feedback models through few-shot examples, known as in-context learning.
We include "transcript - gold summary - reference summary - explanation" tuples as examples for low and high negative impact as context for the feedback model.

The whole prompt is set up as a role definition, few-shot examples, required content such as a reference summary and optional meeting transcript, and the definition of primary tasks (e.g., providing a score) and secondary tasks (e.g., reasoning, confidence, etc.).
All feedback models are given the same prompt structure with adjusted error description and example.

We use two different prompting methods:
\begin{itemize}
    \item \textbf{Direct prompting} prompts for a binary Yes/No output for every error. The model must either output if a respective error occurs ('Yes') or not ('No').
    \item  \textbf{CoT prompting} is an extension of the direct prompting. Instead of a pure binary response, we task the model to explain why it considers a text passage as erroneous. The model should thereby provide reasoning for all errors according to an error type that the model defines throughout the whole text.
\end{itemize}

The result of the error identification is a consolidated list of what errors occurred in detail.
This list is then transferred to the refiner module.




\subsection{Feedback Paradigm}
The feedback format can be dynamic in length and level of detail.
The basic feedback is a Likert score similar to the human assessment applied for the DATASET creation, which assesses either the existence through Yes/No or the quality impact from 1 minimal impact to 5 high impact.

Additionally, we can provide feedback on for each \textit{individual} error regarding error location, reasoning, certainty, correction, and severity.
\begin{itemize}
    \item error location: <details HOW exactly the error location looks like>
    \item correction:
    \item reasoning: 
    \item severity:
    \item certainty: <details HOW exactly the error location looks like>
\end{itemize}


transfer of feedback
\begin{itemize}
    \item A
    \item B
    \item C
\end{itemize}


inclusion of feedback
\begin{itemize}
    \item A
    \item B
    \item C
\end{itemize}
The refiner module is prompted to include the feedback and change the original summary accordingly.




==> text/archive/05_Experiments.tex <==
In this section, we explore the different set-ups possible with the feedback-refinement architecture.
We employ both automatic metrics and human assessment to evaluate the quality, faithfulness, and controllability of the generated summaries.

\subsection{Experiment Settings}

\paragraph{Dataset.}

\paragraph{Models.}

\paragraph{Evaluation metrics.}

\subsection{Baselines}
\paragraph{(Single) Models.}
\paragraph{Prompting approaches.}

\input{figures/callables/RQ2_template_result}


\subsection{RQ1: Can LLMs find summarization-related mistakes (pre-defined) in automatically generated dialogue summaries?}
\begin{itemize}
    \item How do we prompt an LLM (or ensemble) to identify a mistake? --> How reliable is the identification?
    \item What is the most effective way to identify summarization-related mistakes (single model, ensemble, …) --> Which errors can be detected?
\end{itemize}
\noindent \textbf{Approach.}

\noindent \textbf{Observation.}

\noindent \textbf{Discussion.}

\subsection{RQ2: Can an LLM be prompted to correct the summary and thereby improve its quality after it is provided with feedback on the mistakes?}
\begin{itemize}
    \item How does the refinement based on the feedback impact the quality? --> How should the protocol be designed? (1. level of detail, 2. presentation of feedback, 3. feedback incorporation, 4. number of iterations)
\end{itemize}

\noindent \textbf{Approach.}

\noindent \textbf{Observation.}

\noindent \textbf{Discussion.}

\subsection{RQ3: Can the feedback identification and refinement be improved by applying multi-agent discussion?}
\begin{itemize}
    \item What if we have more refiners to discuss the feedback inclusion?
\end{itemize}
\noindent \textbf{Approach.}
Motivation: Why should discussion improve this in the first place? What is the motivation behind this thought?

\noindent \textbf{Observation.}

\noindent \textbf{Discussion.}


\subsection{Scenario 1: What are the influences of model size on the feedback system and refiner performance? (For best performing setup)}
\noindent \textbf{Approach.}
Comparison with Phi 3 (mini)
\noindent \textbf{Observation.}

\noindent \textbf{Discussion.}

\subsection{Scenario 2: How short/long can the feedback be? (For best performing setup)}
\noindent \textbf{Approach.}
different maximum lengths, such as 100, 500, 1000, 2000 tokens
\noindent \textbf{Observation.}

\noindent \textbf{Discussion.}

\subsection{Scenario 3: How does the approach generalize across other conversation types?}
\noindent \textbf{Approach.}
e.g., medic, customer service, ???
\noindent \textbf{Observation.}

\noindent \textbf{Discussion.}



\subsection{RQ4: How does the integration of a feedback loop system impact the quality of generated summaries? Does context, feedback, and target summary length correlate with the overall task performance?}
\input{figures/callables/RQ4_sample_result}

\noindent \textbf{Approach.}

\noindent \textbf{Observation.}

\noindent \textbf{Discussion.}

\subsection{RQ5: Can the feedback identification and refinement be improved by applying multi-agent discussion?}
\noindent \textbf{Approach.}

\noindent \textbf{Observation.}

\noindent \textbf{Discussion.}

\subsection{Use Case Scenario: What are the influences of model size on the feedback system and refiner performance?}
\noindent \textbf{Approach.}

\noindent \textbf{Observation.}

\noindent \textbf{Discussion.}
